RoboBrain: Large-Scale Knowledge Engine for Robots

In this paper we introduce a knowledge engine, which learns and shares knowledge representations, for robots to carry out a variety of tasks. Building such an engine brings with it the challenge of dealing with multiple data modalities including symbols, natural language, haptic senses, robot trajectories, visual features and many others. The \textit{knowledge} stored in the engine comes from multiple sources including physical interactions that robots have while performing tasks (perception, planning and control), knowledge bases from the Internet and learned representations from several robotics research groups. We discuss various technical aspects and associated challenges such as modeling the correctness of knowledge, inferring latent information and formulating different robotic tasks as queries to the knowledge engine. We describe the system architecture and how it supports different mechanisms for users and robots to interact with the engine. Finally, we demonstrate its use in three important research areas: grounding natural language, perception, and planning, which are the key building blocks for many robotic tasks. This knowledge engine is a collaborative effort and we call it RoboBrain.

==> crowdsourcing.tex <==
% !TEX root = robobrain.tex

\section{Crowdsourcing}

One key component in RoboBrain is the use of crowd-sourcing.   While 
previous works have focussed on using crowd-sourcing for data collection and
labeling (e.g., \cite{blah,blah2}), our work focusses on taking crowd-sourced
feedback at many levels:
\begin{itemize}

\item \emph{Weak feedback.}  We have found that it is easiest for users
to provide a binary ``Approve''/``Dispprove'' feedback while they are browsing
online. Our RoboBrain system encourages users to provide such feedback
which is used for  several purposes such as estimating the belief on the nodes
and edges in RoboBrain.

% \todo{Talk about feedback on feeds.}

\item \emph{Feedback on graph.}  We present the graph to the users on the Internet
and smartphones, where they can give feedback on the correctness of a node
or an edge in the graph.  Such feedback is stored for inferring the latent graph.
The key novelty here is that the system shows the proposed ``learned" concepts to the 
users --- thus getting feedback not at the data level but at the knowledge level.

% \todo{Feedback directly on graph.}

\item  \emph{Feedback from partner projects.}   There are several partner 
projects to RoboBrain, such as Tell Me Dave, PlanIt, and so on.  These projects
have a crowd-sourced system where they take feedback, demonstrations,
or interaction data from the users. Such data as well as the learned knowledge 
could be shared with RoboBrain.

% \todo{Feedback via partner projects individual crowd-sourcing. (RoboBrain is a meta-effort.)}

\end{itemize}


==> properties.tex <==
% !TEX root = robobrain.tex


